End-to-end Learning for Graph Decomposition

We propose a novel end-to-end trainable framework for the graph decomposition problem. The minimum cost multicut problem is first converted to an unconstrained binary cubic formulation where cycle consistency constraints are incorporated into the objective function. The new optimization problem can be viewed as a Conditional Random Field (CRF) in which the random variables are associated with the binary edge labels of the initial graph and the hard constraints are introduced in the CRF as high-order potentials. The parameters of a standard Neural Network and the fully differentiable CRF are optimized in an end-to-end manner. Furthermore, our method utilizes the cycle constraints as meta-supervisory signals during the learning of the deep feature representations by taking the dependencies between the output random variables into account. We present analyses of the end-to-end learned representations, showing the impact of the joint training, on the task of clustering images of MNIST. We also validate the effectiveness of our approach both for the feature learning and the final clustering on the challenging task of real-world multi-person pose estimation.

==> chapters/appendices.tex <==
\section{Appendix}

\subsection{Network Architecture for Multi-person Pose Estimation}
In this section, we explain the network architecture and training scheme in details for the application of multi-person pose estimation. The network for pose estimation also consists of four parts:
1) a front end CNN, built based on the architecture of Cao et al.~\citep{cao2017realtime} that outputs feature representations for body joints and limbs; 2) two fully connected layers to convert the features to the unary potentials of the CRF model; 3) a stack of customized layers that perform the iterative mean field updates with high-order potentials; and 4) a standard cross entropy layer to penalize the predicted edge label that is inconsistent with the ground truth label.

\subsubsection{From CNN to Unary Potentials}
\label{sec:unary_pose}

\myparagraph{Front-end CNN.}
Recent work \cite{he2017mask,pishchulin2016deepcut,cao2017realtime,insafutdinov-2017} has made significant progress on multi-person pose estimation by the driving force of deep feature learning. 
%
For instance, the work proposed by Cao et al.~\cite{cao2017realtime} presents an effective deep neural network to learn feature representation for body joints and limbs, followed by a fast heuristic matching algorithm to associate body joints to individual pose. We utilize their  network architecture as the front end CNN. Our model is complementary to this work in the way that our focus is the joint optimization of the deep feature learning and the detection association.  The network proposed in \cite{cao2017realtime} has two separate branches after sharing several convolutional layers: one branch predicts the confidence maps for body joints and the other branch estimates a set of part affinity fields, which encode joint to joint relations.
%
The part field is a 2D vector field. More specifically, each pixel in the affinity field is associated with an estimated 2D vector that encodes the direction pointing from one joint to the other. In \cite{cao2017realtime}, the part fields are built only for pairs of joints that follow the kinematic tree of the human body, e.g. left elbow to left hand. However, in order to incorporate high order potentials among neighboring joints, we train the model to also capture the feature between jump connections, e.g. shoulder to wrist.

% We follow this design as it is nonintuitive and probably difficult to learn robust part fields for pairs of nonadjacent joints, e.g. head to knee.
%

\myparagraph{Graph Construction.} Given an input image, we first obtain the body joint candidates from the detection confidence maps. For each type of the joint, we keep multiple detection hypotheses even for those that are in close proximity. A detection graph is then constructed in the way that we insert edges for pairs of hypotheses that describe the same type of body joint, and for pairs of hypotheses between two different joints. Note that, although the constructed graph is not fully connected, every chordless cycle in the graph consists of only three edges. 
% follow the kinematic tree and also

\myparagraph{Edge Feature.} One of the keys to robust graph decomposition is a reliable feature representation on the edges to indicate whether the corresponding joint detections belong to the same/different person. For the edges that connect the detection hypotheses of different body types, the corresponding part field estimation is utilized as features. More specifically, we compute the inner product between the unit vector defined by the direction of the edge and vectors estimated by the part field. We collect a constant number of values by uniformly sampling along the line segment defined by the edge to form the feature $f_e$ for the corresponding edge. For the edges connecting the detection hypotheses of the same joint type, we simply use the euclidean distance between the detection as the feature.

% A better way would be to design another branch for the network \cite{cao2017realtime} to predict whether the two detections of the same joint type describe the same person; we leave this for future work.

\myparagraph{The Unary $\psi^{U}$.} It is straightforward to construct the unary potentials $\psi_{i}^{U}(x_{i})$ (Eq.~\ref{eq:crf-general}) from the edge feature $f_e$. We incorporate several fully connected layers to encode the feature to classify if an edge is cut, namely, the two corresponding joints belong to different persons. 
As described in Sec.~\ref{sec:CRF}, during training, we can obtain the error signal from the mean field updates to learn the parameters of the newly introduced fully connected layers and the front end CNN that produces the edge feature.

\subsubsection{Mean Field Updates}
\label{sec:mean_Field_update}
Zheng et al.~\cite{Zheng:2015:CRF:2919332.2919659} propose to formulate the mean field iteration as recurrent neural network layers, and ~\cite{Arnab2016HigherOC} further extend it to include high-order object detection and superpixel potentials for the task of semantic segmentation. In this work, we follow their framework with the modification of incorporating our pattern-based potentials.
The goal of the mean field iterations is to update the marginal distribution  $Q^{t}_{i}(x_i = l)$. For initialization, $Q^{1}_{i}(x_i = l) = \frac{1}{Z_i} \exp\{-\psi_{i}^{U}(x_{i}=l)\}$, where $Z_i = \sum_l \exp\{-\psi_{i}^{U},(x_{i}=l)\}$ is performed. This is equivalent to applying a soft-max function over the negative unary energy across all the possible labels for each link. This operation does not include any parameters and the error can be back-propagated to the front end convolutional or fully connected layers where the unary potentials come from. Once the marginal has been initialized, we compute the high order potentials based on Eq.~\eqref{eq:mean-field-update-ours}. Specifically, the valid cliques in $\mathcal{P}_{c}$ are 0-0-0, 1-1-1 and 1-1-0, while the non-valid cliques are 0-0-1, where 1 indicates that the corresponding edge is cut. This operation is differentiable with respect to the parameters $\gamma_{\mathbf{x}_{c}}$ and $\gamma_{max}$ introduced in Eq.~\eqref{eq:mean-field-update-ours}, allowing us to optimize them via backpropagation. The errors can also flow back to  $Q^{1}(X)$. Once the high order potential is obtained, it is summed up with the unary potential and then the sum is normalized via the soft-max function to generate the new marginal for the next iteration. Multiple mean-field iterations can be efficiently implemented by stacking this basic operation. During the inference, as the mean field inference does not guarantee a feasible solution to the original optimization problem, we use the fast heuristic proposed in \cite{cao2017realtime} as an additional step to come back to the feasible set. 

\subsubsection{Loss and Training}
\label{sec:loss}
During training, we first train the joint confidence maps and part affinity field maps with  a standard $L2$ loss as described in~\cite{cao2017realtime}. Once the basic features are learned, the next step is to train the unary with the softmax loss function. This is performed in an on-the-fly manner, which means the detection hypotheses for the body joints are estimated and then the links between the hypotheses are also established during training time. Their ground-truth labels are also generated online at the same time. The final step is to train the parameters of the CRF with high order potentials with a softmax loss function in an end-to-end manner along with the basic convolutional and fully connected layers.

==> chapters/experiments.tex <==
\section{Experiments}

In this section, we evaluate our proposed end-to-end learnable solution for the graph decomposition problem on the challenging multi-person pose estimation task. 
%
We first demonstrate the effectiveness of the proposed CRF model for updating the marginals based on the high-order potentials.
%
Then we measure the ratio of validity for the cycle constraints before and after the mean field inference iterations. 
%
The influence of the end-to-end learning on the feature representation learning and the final pose association will also be discussed.

\myparagraph{Dataset.}
MPII Human Pose dataset consists of about 25k images and contains around 40k total annotated people. 
%
There is a training and test split with 3844 and 1758 groups of people respectively. 
We conduct ablation experiments on a held out validation set. 
%
During testing, no information about the number of people or the scales of individual is provided. 
%
For the final association evaluation, we deploy the evaluation metric proposed by Pishchulin et al.~\cite{pishchulin2016deepcut}, calculating the average precision of the joint detections for all the people in the images. In the following experiments, we use shortcuts for body joints (Head-H, Shoulder-S, Elbow-E, Wrist-W, Hip-Hi, Knee-K, Ankle-A).


\begin{figure}[t!]
	\includegraphics[width=\textwidth]{figures/PF_update.png}
    \caption{\textbf{Feature learning comparison.} Left: input image; Middle: part field map without CRF inference; Right: part field map after inference (Only arms and legs shown). The samples in the \textbf{top two rows} show sharper and more accurate confidence maps. The fist example in the \textbf{last row} shows that, for the non-overlapping case, the original network is already very precise, while the \textbf{last example} is a failure case where the CNN does not capture any features on the right side of the image.}
    \label{fig:part-field map}
\end{figure}

\myparagraph{Implementation Details.}
The front-end CNN architecture has several stacked fully convolutional layers with an input size of 368x368 as described in \cite{cao2017realtime}. We train the basic CNN using a batch size of 12 with a learning rate of 1e-4. 
For training the CRF parameters, the learning rate is 1e-5. 
The whole architecture is implemented in Caffe~\cite{jia2014caffe}.

\myparagraph{Effectiveness of the CRF Inference.}
To demonstrate the effectiveness of our proposed mean-field layers approximating the CRF inference, we evaluate the evolution of the marginal distribution for the random variables $X$.
%
For pose estimation, each variable $X_i$ in the CRF represents a link between two body joints. 
As seen in Tab.~\ref{table:marginal}, 7 different types of limbs are depicted. 
%
The numbers are the average marginal probabilities for those links with the ground truth of not being cut. 
This index measures how confident a link is supposed to be associated, namely, the two body joints belong to the same person.
%
As shown in the table, the marginal distributions of all the limbs benefit from high order potentials even for the conventionally challenging ones, e.g. Elbo-Wris and Knee-Ankl. After three iterations of the mean field inference, the update is converged so we fix this setting for other experiments.
% The values in the brackets represent the links with ground truth of cut.

\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccccccc}
\hline
 & Head-Neck &Neck-Shou  & Shou-Elbo &Elbo-Wris &Shou-Hip &Hip-Knee &Knee-Ankl  & Mean \\
\hline
 origin &  0.755 & 0.656 & 0.662 & 0.558& 0.679& 0.593 & 0.611& 0.635 \\
\hline
 Iter 1&   0.783 & 0.692 & 0.688 & 0.579& 0.711& 0.628 & 0.639& 0.659 \\
 Iter 2&   0.805 & 0.707 & 0.715 & 0.603& 0.726& 0.649 & 0.651& 0.671 \\
 Iter 3&   0.807 & 0.712 & 0.716 & 0.608& 0.723& 0.646 & 0.653& 0.674 \\

\hline
\end{tabular}
}
\end{center}
\vspace{-0.5em}
\caption{\textbf{Marginal distribution updates.} Numbers represent evolution of the marginal probabilities along with the mean-field iterations for different type of limbs.} %The samples are with ground truth of link.}
\label{table:marginal}
\vspace{-1em}
\end{table}


\myparagraph{Validity of the Cycle Constraints.}
Another important measurement for our proposed model is to check the ratio of non-valid cycles before and after the mean field iterations. 
%
% We set the threshold of cut to 0.5, which means if the probability is below 0.5, we cut the link.
%
As mentioned in Sec.~\ref{sec:end-to-end learning}, the type of non-valid 3-clique is link-link-cut. We can see from Tab.~\ref{table:non valid cycle} that, with the CRF inference, the ratios of non-valid cycles are reduced, which indicates the effectiveness of the high order potential.

\begin{table}
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\hline
 & Head-Neck-Shou  & Shou-Elbo-Wris  &Neck-LHip-RHip &Hip-Knee-Ankl & Mean \\
\hline
 origin &  1.68 & 3.40 & 1.41 & 3.83& 2.60  \\
 \hline
 Iter 1&   1.12 & 2.79 & 1.06 & 3.17& 2.04  \\
 Iter 2&   1.01 & 2.58 & 0.89 & 2.82& 1.81 \\
 Iter 3&   0.96 & 2.47 & 0.87 & 2.79& 1.76 \\
\hline
\end{tabular}
}
\vspace{-0.5em}
\caption{\textbf{Ratio of non valid cycle.} Numbers (\%) represent the ratio of non valid cycle for four different types of cliques that are defined for adjacent body joints.}
\vspace{-2em}
\label{table:non valid cycle}
\end{table}



\myparagraph{Benefit of End-to-End Learning on Feature Representation.}
One of the key advantages of training the CNN and CRF in a unified framework is to obtain a better feature representation. 
%
% The improvement on the marginal distributions (as shown in Tab.~\ref{table:marginal}) has implicitly indicated 
% that, by the end-to-end learning, the deep feature representation of the front end CNN is steadily improved.
We illustrate it by directly visualizing the part field feature maps before and after the mean field inference.
%
As shown in the top two rows of Fig.~\ref{fig:part-field map}, the part field confidence maps in general get sharper and cleaner, particularly for images with heavy occlusions; e.g.~in the second image in the second row, the limbs of the partially occluded people become much more distinguishable, suggesting a notable improvement in the feature learning for the challenging cases. 
%
This is in line with one of the assumptions of this work: the training of the deep features needs additional supervision signals from the high-order terms, particularly for challenging cases.
% because these terms guide the network training by taking the dependencies between the output random variables into account.
%
The fist example in the last row shows a non-overlapping case. Not surprisingly, the features that are learned with and without high-order information are equally informative.
% For the non-occlusion cases, e.g. the fist example in the last row
% The fist example in the last row shows that for the non-overlapping case the original training with $L_2$ loss can already capture features very accurately. 
%
% However, for groups of people with heavy overlapping, the feature learning is still very tough even with CRF inference. 
%
The last example in the last row is a failure case where the end-to-end learning does not help significantly. 
This might be due to shadows and relative scale differences.



\myparagraph{Return to a Feasible Solution.}
\begin{figure}
	\includegraphics[width=1\textwidth]{figures/association_new.png}
    \caption{\textbf{Qualitative Results.}  Left: association  without CRF inference; Right: association after inference. \textbf{First row}, obvious wrong connections are corrected by inference. In the \textbf{second row} occluded people are separated. The samples in the \textbf{last row} are failure cases.}
    \label{fig:association}
\end{figure}
After the CRF inference, we do not obtain a valid graph decomposition directly. Some heuristics (either the greedy search~\cite{cao2017realtime} or the Kernighan-Lin (KL) heuristic~\cite{insafutdinov-2017}) are required to generate a valid decomposition efficiently. We evaluate these two heuristics with three different settings for each: 1) only front-end CNN and full connected layers (unary); 2) trained CRF on top of front-end CNN and fully connected layers (unary and CRF); 3) end-to-end finetuning of the whole network ( end-to-end finetuning).

Tab.~\ref{table:c} shows the analysis on the validation set and we can see the advantage of the
end-to-end strategy over the offline training of CRF as a
post-processing method. As illustrated in Fig.~\ref{fig:association}, the improvements are mainly achieved on the challenging cases with heavy occlusion, which benefit from modeling the high-order dependency among the variables of interest.
Overall, based on the same front-end CNN, the greedy search~\cite{cao2017realtime} outperforms the KL heuristic~\cite{insafutdinov-2017}. Our intuitions are as follows: we construct the graph by considering pairs of joints that follow the kinematic tree of the human body and pairs of joints between jump connections, e.g. shoulder to wrist. The part field for the pairs of joints between jump connections are not as good as the ones for the pairs of joints that follow the kinematic tree (also stated in~\cite{cao2017realtime}). The KL heuristic uses all types of connections to perform the graph decomposition whereas the greedy search ~\cite{cao2017realtime} only considers the kinematic tree. As a result, the greedy search~\cite{cao2017realtime} is potentially affected less by the undesired part affinity. 

\begin{table}
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccccc|c}
\hline
 Method& Head & Shou &Elbo &Wris &Hip &Knee &Ankl &Mean \\
\hline
unary (KL~\cite{insafutdinov-2017})& 88.55  &  83.98 & 71.43  & 60.97  & 73.44  & 65.25 & 56.66 & 71.32 \\
unary and CRF (KL~\cite{insafutdinov-2017}) & 89.04  & 84.36  & 72.01  & 61.39  & 73.68  &66.75  & 58.11 & 71.96 \\
end-to-end finetuning  (KL~\cite{insafutdinov-2017}) &  89.38 & 84.72 & 72.49  & 61.96  &  74.05 &  66.85 & 58.46 & 72.57 \\
unary (greedy ~\cite{cao2017realtime})& 91.30 & 86.14   &  73.69 & 62.84  &  73.40 & 66.43 & 58.73   & 73.21 \\

unary and CRF (greedy~\cite{cao2017realtime})& 91.31 & 86.47  & 74.60  & 64.01 & 73.69 &  66.98& 59.45 & 73.78 \\
end-to-end finetuning  (greedy~\cite{cao2017realtime}) & 91.50 & 86.90   &  74.89 & 64.61  &  73.97 & 67.38 & 59.91 & 74.36 \\
\hline
\end{tabular}
}
%\vspace{-0.3em}
\caption{Multi-person pose estimation result on the validation set. }
\label{table:c}
\vspace{-1em}
\end{table}

\myparagraph{Comparison With Others.}
We test the proposed method on the MPII Human Pose dataset and compare with other methods.
The result are shown in Tab.~\ref{table:c}.
% The baseline of our evaluation is our implementation of \cite{cao2017realtime}, which
% obtaines 75.2 mAP on the test set.
% We use the baseline network as the front end CNN and combine it with the proposed CRF. 
% The overall performance is boosted to 75.9 mAP, which is on par with other state-of-the-art methods.
Our end-to-end method achieves 76.1 mAP, which is on par with other state-of-the-art methods.
Note that the method proposed in \cite{newell2017associative} uses a single-person pose estimator to refine the final result, and \cite{fang2017rmpe} is a top-down method where a Faster R-CNN \cite{Ren:2015:FRT:2969239.2969250} person detector is utilized. 
\vspace{-1em}
\begin{table}
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccccc|c}
\hline
 Method& Head & Shou &Elbo &Wris &Hip &Knee &Ankl &Mean \\
\hline
Iqbal et al., \cite{iqbal2016multi} & 58.4  & 53.9  & 44.5  & 35.0  & 42.2  & 36.7 & 31.1 & 43.1 \\
pishchulin et al., \cite{pishchulin2016deepcut}& 89.4  & 84.5  & 70.4  & 59.3  & 68.9  & 62.7 & 54.6 & 70.0 \\
Insafutdinov et al., \cite{insafutdinov-2016}& 78.4  & 72.5  & 60.2  & 51.0  & 57.2  & 52.0 & 45.4 & 59.5 \\
Insafutdinov et al., \cite{insafutdinov-2017}& 88.8  & 87.0  & 75.9  & 64.9  & 74.2  & 68.8 & 60.5 & 74.3 \\

Cao et al., \cite{cao2017realtime}& 91.2  & 87.6  & 77.7  & 66.8  & 75.4  & 68.9 & 61.7 & 75.6 \\
Fang et al., \cite{fang2017rmpe}& 88.4  & 86.5  & 78.6  & 70.4  & 74.4  & 73.0 & 65.8 & 76.7 \\
Newell et al., \cite{newell2017associative}& 92.1  & 89.3  & 78.9  & 69.8  & 76.2  & 71.6 & 64.7 & 77.5 \\
Nie et al., \cite{nie2018pose}& 92.2  & 89.7  & 82.1  & 74.4  & 78.6  & 76.4 & 69.3 & 80.4 \\
\hline
% Baseline & 90.7  & 87.4 & 77.3 & 66.5  &75.7 & 69.0 &60.9 & 75.2 \\
Our Method & 91.4 & 87.8  & 78.0  & 67.2  &76.5 & 69.3 &62.2 & 76.1 \\
% 3-iters & 97.0 & 87.3 &74.9 &71.1 &97.5 &89.4 &86.0& 86.9\\
% 3-iters & 97.1 & 95.7 &87.5 &81.6 &98.0 &92.7 &89.8& 92.1\\
\hline
\end{tabular}
}
\vspace{-0.3em}
\caption{Comparison with the state-of-the-art on the MPII Human Pose dataset.}
\label{table:c}
\vspace{-2em}
\end{table}

% As discussed in Sec.~\ref{sec:related}, the multi-person pose estimation works can be categorized as top-down based (from person detection to individual poses) or bottom-up based methods (from body joint detections to individual poses).
% The top-down methods currently get superior performance mainly because of the robustness of person detectors that are trained on a large amount of training examples.
% In contrast, the bottom-up based methods require the annotation of body joints, which are much more difficult to obtain. 
% %Bottom-up based methods suffer from lack of training data. 
% The training error of the CNN in \cite{cao2017realtime} is close to zero, suggesting a model over-fitting. When we add the CRF layers on top of the CNN to jointly learn the deep features and the high-order relations, the over-fitting of the training becomes even more severe. 

% Our model is aiming to jointly learn the appearance features and also multiple
% pose relationship, which is a complicated/high dimensional configuration space. Due to the
% difficulty of accurate annotation, the current dataset is still limited to learn this configuration,
% especially for those highly crowded and occluded cases.



% \myparagraph{Qualitative Results}
% In Fig.~\ref{fig:association}, the final association results are compared between the model without (left) and with (right) the end-to-end mean field inference. For the samples in the first row, obvious wrong connections are corrected by high order potentials. The second row shows that highly occluded people are correctly separated by our proposed model. The samples in the last row are failure cases. One is because of heavy occlusion among a group of people with rare poses, and the other is mainly because of the scale of the person.
% \begin{figure}
% 	\includegraphics[width=\textwidth]{figures/part_field_new.png}
%     \vspace{-2em}
%     \caption{\textbf{Feature learning comparison.} Left: input image; Middle: part field map without CRF inference; Right: part field map after inference (Only arms and legs shown). The samples in the \textbf{top two rows} show sharper and more accurate confidence maps. The fist example in the \textbf{last row} shows that, for the non-overlapping case, the original network is already very precise, while the \textbf{last example} is a failure case where the CNN does not capture any features on the right side of the image.}
%     \label{fig:part-field map}
% \end{figure}

% \begin{figure}
% 	\includegraphics[width=1\textwidth]{figures/association_new.png}
%     \vspace{-2em}
%     \caption{\textbf{Qualitative Results.}  Left: association  without CRF inference; Right: association after inference. \textbf{First row}, obvious wrong connections are corrected by inference. In the \textbf{second row} occluded people are separated. The samples in the \textbf{last row} are failure cases.}
%     \label{fig:association}
% \end{figure}


